Plane algebraic curves with prescribed singularities

We report on the problem of the existence of complex and real algebraic curves in the plane with prescribed singularities up to analytic and topological equivalence. The question is whether, for a given positive integer $d$ and a finite number of given analytic or topological singularity types, there exist a plane (irreducible) curve of degree $d$ having singular points of the given type as its only singularities. The set of all such curves is a quasi-projective variety, which we call an equisingular family (ESF). We describe, in terms of numerical invariants of the curves and their singularities, the state of the art concerning necessary and sufficient conditions for the non-emptiness and $T$-smoothness (i.e., smooth of expected dimension) of the corresponding ESF. The considered singularities can be arbitrary, but we spend special attention to plane curves with nodes and cusps, the most studied case, where still no complete answer is known in general. An important result is, however, that the necessary and the sufficient conditions show the same asymptotics for $T$-smooth equisingular families if the degree goes to infinity.

==> ref.tex <==


\begin{thebibliography}{99.}
\bibitem{AM} Abhyankar, S. S., Moh, T. T.: %Newton-Puiseux expansion and generalized Tschirnhausen transformation, I. J. reine angew. Math. {\bf260}, 47--83 (1973)
      Embeddings of the line in the plane. J. Reine Angew. Math. {\bf 276}, 148--166 (1975)
\bibitem{AC} A'Campo, H.: Le groupe de monodromie des singularit\'es isol\'ees des courbes planes, I.
Math. Ann. {\bf 213}, 1--32 (1975)
\bibitem{AG} Akyol, A., Degtyarev, A.: Geography of irreducible plane sextics. Proc. Lond. Math. Soc. (3)
{\bf111}, no. 6, 1307--1337 (2015)
\bibitem{AH1} Alexander, J., Hirschowitz, A.: An asymptotic vanishing theorem for generic unions of multiple points. Invent. Math. {\bf 140}, no. 2, 303--325 (2000)
\bibitem{BK} Brieskorn, E., Kn\"orrer, H.: Plane algebraic curves.
Birkh\"auser-Verlag, Switzerland (1986)
%\bibitem{Bru}
%Bruce, J. W.: An upper bound for the number of singularities on a projective hypersurface.
%Bull. Lond. Math. Soc. {\bf 13}, 47--50 (1981)
\bibitem{BG} Bruce, J. W., Giblin, P. J.:
A stratification of the space of plane quartic curves.
Proc. London Math. Soc. {\bf 42}, 270--298 (1981)
\bibitem{Br} Brusotti, L.: Sulla ``piccola variazione" di una
curva piana algebrica reali. Rend. Rom. Ac. Lincei (5) {\bf
30}, 375--379 (1921)
\bibitem{CPS} Calabri, A., Paccagnan, D., Stagnaro, E.: Plane algebraic curves with many cusps with
an appendix by Eugenii Shustin. Annali di Matematica Pura ed Applicata (4) {\bf193}, no. 3, 909--921 (2014)
\bibitem{Ca} Castelnuovo, G.: Ricerche di geometria sulle curve algebriche. Atti Reale Accademia delle Scienze di Torino {\bf 24}, 346--373 (1889)
\bibitem{XiChen} Chen, Xi: Rational curves on K3 surfaces. J. Alg. Geom. {\bf 8}, 245--278 (1999)
\bibitem{XiChen1} Chen, Xi: Nodal Curves on K3 Surfaces. New York J. Math. {\bf 25}, 168--173 (2019)
\bibitem{CNL} Cassou-Nogues, P., Luengo, I.: On $A_k$ singularities on plane curves of fixed degree.
Preprint (2000)
\bibitem{CC} Chiantini, L., Ciliberto, C.: On the Severi varieties of surfaces in $\PP^3$.
J. Alg. Geom. {\bf8}, no. 1, 67--83 (1999)
%\bibitem{CS} Chiantini, L., Sernesi, E.: Nodal curves on surfaces of general type.
%Math. Ann. {\bf 307}, 41--56 (1997)
\bibitem{DGPS} Decker, W., Greuel, G.-M., Pfister, G., Sch\"onemann, H.: Singular 4-1-1 -- A computeralgebra system for polynomial computations (2018). https://www.singular.uni-kl.de 
\bibitem{De1} Degtyarev, A.:
Isotopic classification of complex plane projective curves of degree 5.
Algebra i Analiz {\bf 1}, no. 4, 78--101 (1989)
\bibitem{De2} Degtyarev, A.: Topology of algebraic curves. An approach via dessins d'enfants. Walter de Gruyter,
Berlin/Boston (2012)
\bibitem{DPW} Du Plessis, A. A., Wall, C. T. C.: Singular hypersurfaces, versality and Gorenstein algebras.
J. Algebraic Geom. {\bf9}, no. 2, 309--322 (2000)
\bibitem{FPST} Fomin, S., Pylyavskyy, P., Shustin, E., Thurston, D.:  Morsifications and mutations. Preprint at arXiv:1711.10598.
\bibitem{FP} Fulton, W., Pandharipande, R. Notes on stable maps and quantum cohomology. Algebraic geometry---Santa Cruz 1995, Proc. Sympos. Pure Math., 62, Part 2, Amer. Math. Soc., Providence, RI, pp. 45--96 (1997)
%\bibitem{GD} Giacinti-Diebolt, C.: Vari\'et\'es des courbes projectives
%planes de degr\'ee et lieu singulier donn\'es. Math. Ann. {\bf 266}, no. 3, 321--350 (1984)
\bibitem{Gou} Gourevich, A. Geometry of obstructed families of curves. J. Pure Appl. Algebra {\bf210}, no. 3, 721--734 (2007)
\bibitem{GP} G\"ottsche, L., Pandharipande, R.: The quantum cohomology of blow-ups of $\PP^2$ and enumerative geometry. J. Differential Geom. {\bf48}, no. 1, 61--90 (1998)
%\bibitem{GM1} Gradolato, M., Mezzetti, E.: Curves with nodes, cusps
%and ordinary triple points.  Ann. Univ. Ferrara, sez. 7,
%{\bf 31}, 23--47 (1985)
%\bibitem{GM2} Gradolato, M. A., Mezzetti, E.:
%Families of curves with ordinary singular points on regular surfaces.
%Ann. mat. pura ed appl. {\bf 150}, 281--298 (1988)
%\bibitem{G} Greuel, G.-M.: A remark on the paper of A.\ Tannenbaum. Compos. Math.\ {\bf 51},
%185--187 (1984).
\bibitem{GK} Greuel, G.-M., Karras, U.: Families of varieties with
prescribed singularities. Compos. Math. {\bf 69}, no. 1, 83--110 (1989)
\bibitem{GL} Greuel, G.-M., Lossen, C.:
Equianalytic and equisingular families of curves on surfaces.
Manuscr.\ Math. {\bf 91}, 323--342 (1996)
\bibitem{GLS0} Greuel, G.-M., Lossen, C., Shustin, E.: New asymptotics in the geometry of equisingularfamilies of curves. Int. Math. Res. Not. {\bf13}, 595--611 (1997)
\bibitem{GLS1} Greuel G.-M., Lossen, C., Shustin, E.:
Plane curves of minimal degree with prescribed singularities.
Invent. Math. {\bf 133}, no. 3, 539--580 (1998)
\bibitem{GLS2} Greuel, G.-M., Lossen, C., Shustin, E.:
Families of nodal curves on the blown-up projective plane.
Trans. Amer. Math. Soc. {\bf 350}, no. 1, 251--274 (1998)
\bibitem{GLS5} Greuel, G.-M., Lossen, C., Shustin, E.: Castelnuovo function, zero-dimensional schemes and singular plane curves. J. Algebr. Geom. {\bf9}, no. 4, 663--710 (2000)
\bibitem{GLS4} Greuel, G.-M., Lossen, C., Shustin, E.: The Variety of Plane Curves with Ordinary Singularities is not irreducible. Intern. Math. Res. Notices {\bf 11}, 542--550 (2001)
\bibitem{GLS-ISD} Greuel, G.-M., Lossen, C., Shustin, E.: Introduction to singularities and deformations. Springer, Berlin (2007)
\bibitem{GLS3} Greuel, G.-M., Lossen, C., Shustin, E.: Singular algebraic curves. Springer, Switzerland (2018)
%\bibitem{GPS} Greuel, G.-M., Pfister, G., Sch\"onemann, H.: SINGULAR,
%    A Computeralgebra system for Algebraic Geometry and Singularity theory.
%  Available via ftp from helios.mathematik.uni-kl.de.
\bibitem{GH} Griffiths, P., Harris, J.: Principles of algebraic geometry. John Wiley, NY (1978)
\bibitem{Gu} Gudkov, D. A.: On the curve of 5th order with 5 cusps. Funct. Anal. Appl.
{\bf16}, 201--202 (1982)
\bibitem{Gu1} Gudkov, D. A., Tai, M. L., Utkin, G. A.:
Complete classification of irreducible curves of the 4th order.
Mat. Sbornik {\bf 69}, no. 2, 222--256 (1966)
\bibitem{GZ} Gusein-Zade, S. M.: Dynkin diagrams for singularities of functions of two variables.
Func. Anal. Appl. {\bf 8}, 295--300 (1974)
\bibitem{GZN} Gusein-Zade, S. M., Nekhoroshev, N. N.: Singularities of type $A_k$ on simple curves of chosen degree. Funct. Anal. Appl. {\bf34}, no. 3, 214--215 (2000)
\bibitem{HJ} Harris, J.: On the Severi problem. Invent. Math. {\bf 84}, 445--461 (1985)
\bibitem{HA} Hirano, A.: Constructions of plane curves with cusps.
Saitama Math. J. {\bf 10}, 21--24 (1992)
\bibitem{Hir} Hironaka, H.: On the arithmetic genera and the effective genera of algebraic curves.
Mem. Coll. Sci., Univ. of Kyoto {\bf30}, 177--195 (1957)
\bibitem{HF} Hirzebruch, F.: Singularities of algebraic surfaces
and characteristic numbers. Contemp. Math. {\bf 58}, 141--155 (1986)
\bibitem{IS} Itenberg, I., Shustin, E.: Real algebraic curves with real cusps.
Amer. Math. Soc. Transl. (2) {\bf 173}, 97--109 (1996)
%\bibitem{IS1} Itenberg, I., Shustin, E.: Combinatorial patchworking of real pseudo-holomorphic curves.
%Turkish J. Math. {\bf 26}, no. 1, 27--51 (2002)
\bibitem{Iv} Ivinskis, K.: Normale Fl\"achen und die Miyaoka-Kobayashi Ungleichung.
Diplomarbeit, Bonn (1985)
%\bibitem{K1} Kang, P.-L.: On the variety of plane curves of degree $d$
%with $\del$ nodes and $k$ cusps. Trans. Amer. Math. Soc. {\bf 316}, no. 1,
%165--192 (1989)
%\bibitem{K2} Kang, P.-L.: A note on the variety of plane curves with
%nodes and cusps. Proc. Amer. Math. Soc. {\bf 106}, no. 2, 309--312 (1989)
\bibitem{Ker} Kerner, D.: Recombination formulas for the spectrum of curve singularities and some applications. Preprint at arXiv:1403.5789.
\bibitem{Koe} Koelman, R.~J.: Over de cusp. University of Leiden, Diplomarbeit (1986)
\bibitem{KP1} Koras, M., Palka, K.: The Coolidge-Nagata conjecture. Duke Math. J. {\bf 166}, no. 16, 3085--3145 (2017)
\bibitem{KP2} Koras, M., Palka, K.: Complex planar curves homeomorphic to a line have at most four singular points. Preprint at arXiv:1905.11376.
\bibitem{KW1} Korchagin, A. B., Weinberg, D. A.: The isotopy classification of affine quartic curves. Rocky Mountain J. Math. {\bf32}, no. 1, 255--347 (2002)
\bibitem{KW} Korchagin, A. B., Weinberg, D. A.: Quadric, cubic, and quartic cones.
Rocky Mountain J. Math. {\bf 35}, no. 5, 1627--1656 (2005)
\bibitem{Ku} Kulikov, Vik. S.: The generalized Chisini conjecture.
Proc. Steklov Inst. Math. {\bf241}, no. 2, 110--119 (2003)
\bibitem{Lan} Langer, A.: Logarithmic orbifold Euler numbers of surfaces with applications.
Proc. Lond. Math. Soc. (3) {\bf86}, 358--396 (2003)
\bibitem{Lef} Lefschetz, S.: On the existence of loci with given singularities. Trans. Amer. Math. Soc. {\bf 14}, 23--41 (1913)
\bibitem{LS} Leviant, P., Shustin, E.: Morsifications of real plane curve singularities.
J. Singularities {\bf 18}, 307--328 (2018)
%\bibitem{Li} Lindner, M.: \"Uber Mannigfaltigkeiten ebener Kurven mit Singularit\"aten.
%Arch. Math. {\bf 28}, 603--610 (1977)
%\bibitem{Loes} Loeser, F.: Deformations des courbes planes.
%Seminaire Bourbaki, 1986-87, no. 679, 187--205 (1987)
\bibitem{Lu} Luengo, I.: The $\mu$-constant stratum is not smooth.
Invent. Math. {\bf 90}, 139--152 (1987)
\bibitem{Lu1} Luengo, I.:  On the existence of complete families of projective plane curves, which are obstructed.
J. London Math. Soc. {\bf 2-36}, no. 1, 33--43 (1987)
\bibitem{Mi}  Milnor, J.: Singular points of complex hypersurfaces. Princeton Univ. Press, Princeton (1968).
\bibitem{Miy} Miyaoka, Y.: The maximal number of quotient singularities on surfaces with given numerical invariants.
Math. Ann. {\bf268}, 159--171 (1984)
\bibitem{N1} Newton, I.: Analysis of the properties of cubic curves and their classification by species.
The mathematical papers of Isaac Newton (D.T. Whiteside, ed.), Cambridge Univ. Press, vol. 2, pp. 389--34 (1968)
\bibitem{N2} Newton, I.: Enumeratio linearum tertij ordinis. The mathematical papers of Isaac
Newton (D.T.  Whiteside,  ed.),  Cambridge  Univ. Press, vol. 7, pp. 565--645 (1976)
\bibitem{N3} Newton, I.: The final ``Geometri\ae\ libri duo".
The mathematical papers of Isaac Newton (D.T. Whiteside, ed.), Cambridge Univ. Press, vol. 7, pp. 402--469 (1976)
\bibitem{Nor} Nori, M.: Zariski conjecture and related problems. Ann. Sci. Ec. Norm. Sup.
{\bf4} (16), 305--344 (1983)
\bibitem{Ore} Orevkov, S. Yu.: Some examples of real algebraic and real pseudoholomorphic curves.
{\it Perspectives in Analysis, Geometry, and Topology}. Progress in Mathematics, vol. 296,
pp. 355–387, Birkh\"auser, Basel (2012)
\bibitem{Pe1} Pecker, D.: Simple constructions of algebraic curves with nodes.
Compos. Math. {\bf 87}, 1--4 (1993)
\bibitem{Pe3} Pecker, D.: Note sur la r\'ealit\'e des points doubles des courbes gauches.
C. R. Acad. Sci.Paris, S\'er. I {\bf324}, 807--812 (1997)
\bibitem{Pe2} Pecker, D.: Sur le th\`eor\'eme local de Harnack.
C. R. Acad. Sci. Paris, S\'er. I {\bf 326}, no. 5, 573--576 (1998)
\bibitem{Pe4} Pecker, D.: Sur la r\'ealit\'e des points doubles des courbes gauches. Ann.
Inst. Fourier (Grenoble) {\bf49}, 1439--1452 (1999)
\bibitem{Sa} Sakai, F.: Singularities of Plane Curves.
Geometry of Complex Projective Varieties
(Seminars and Conferences 9), Mediterranian Press, Rende, pp. 257--273 (1993)
\bibitem{Schu} Schulze, M.: A singular 3-1-6 library for computing invariants related to the Gauss-Maninsystem of an isolated hypersurface singularity (2012) (gmssing.lib.)
\bibitem{Segre} Segre, B.: Dei sistemi lineari tangenti ad un qualunque sistema di forme.
Atti Acad. naz. Lincei Rendiconti serie 5, {\bf 33},
182--185 (1924)
\bibitem{Segre2} Segre, B.: Esistenza e dimensione di sistemi continui di curve piane algebriche
con dati caraterri. Atti Acad. naz. Lincei Rendiconti serie 6, {\bf 10},
31--38 (1929)
\bibitem{Se} Severi, F.: Vorlesungen \"uber Algebraische Geometrie (Anhang F).
Leipzig, Teubner (1921)
\bibitem{Sh14} Shustin, E. I.: On invariants of algebraic curve singular points. Math. Notes of Acad. Sci. USSR {\bf34}, 962--963 (1983)
%\bibitem{Sh1} Shustin, E.: New M-curve of the 8th degree.
%Math. Notes of Acad. Sci. USSR {\bf 42}, 606--610 (1987)
\bibitem{Sh2} Shustin, E.: Versal deformations in the space of plane curves of fixed degree.
Func. Anal. Appl. {\bf 21}, 82--84 (1987)
%\bibitem{Sh3} Shustin, E.: Hyperbolic and minimal smoothings of singular points.
%Selecta Math. Sov. {\bf 10}, no.1, 19--25 (1991)
\bibitem{Sh4} Shustin, E.: On manifolds of singular algebraic curves. Selecta Math. Sov.
{\bf 10}, no.1, 27--37 (1991)
\bibitem{Sh6} Shustin, E.: Real plane algebraic curves with prescribed singularities. Topology
{\bf 32}, no. 4, 845--856 (1993)
\bibitem{Sh7} Shustin, E.: Smoothness and irreducibility of varieties of algebraic curves with nodes
and cusps. Bull. Soc. Math. France {\bf 122}, 235--253 (1994)
\bibitem{Sh12} Shustin, E.: Gluing of singular and critical points.
Topology {\bf 37}, no. 1, 195--217 (1998)
\bibitem{Sh2000} Shustin, E.: Lower deformations of isolated hypersurface singularities. St. Petersburg Math. J.
{\bf11}, no. 5, 883--908 (2000)
\bibitem{Sh13} Shustin, E.: Analytic order of singular and critical points.
Trans. Amer. Math. Soc. {\bf 356}, 953--985 (2004)
\bibitem{ST1} Shustin, E., Tyomkin, I.: Patchworking singular algebraic curves, I. Israel J. Math.
{\bf151}, 125--144 (2006)
\bibitem{ShW} Shustin, E., Westenberger, E.: Projective hypersurfaces with many singularities of pre-scribed types.
J. Lond. Math. Soc. (2) {\bf70}, no. 3, 609--624 (2004)
\bibitem{St0} Steenbrink, J. H. M.: Intersection form for quasihomogeneous singularities. Compos. Math.
{\bf 34}, no. 2, 211--223 (1977)
\bibitem{St} Steenbrink, J. H. M.: Semicontinuity of the singularity spectrum. Invent. Math.
{\bf 79}, 557--566 (1985)
\bibitem{Ta-1} Tannenbaum, A.: On the geometric genera of projective curves. Math. Ann. {\bf240},
no. 3, 213--221 (1979)
\bibitem{Ta1} Tannenbaum, A.: Families of algebraic curves with nodes.
Compos. Math. {\bf 41}, 107--126 (1980)
\bibitem{Ta2} Tannenbaum, A.: Families of curves with nodes on K3 surfaces.
Math. Ann. {\bf 260}, 239--253 (1982)
\bibitem{Ta0} Tannenbaum, A.: On the classical characteristic linear series of plane curves
with nodes and cuspidal points: two examples of Beniamino Segre.
Compositio Math. {\bf 51}, 169--183 (1984)
\bibitem{Te} Teissier, B.: The hunting of invariants in the geometry of discriminants.
Real and Complex Singularities (P.Holm, ed.), Oslo.
Sijthoff-Noordhoff Publ., Alphen aan den Rijn, pp. 565--677 (1977)
%\bibitem{To} Tono, K.: On the number of the cusps of cuspidal plane curves. Math.  Nachr. {\bf278}, 216--221 (2005)
\bibitem{U1} Urabe, T.: On quartic surfaces and sextic curves with certain singularities.
Proc. Japan. Acad. Ser. A. {\bf 59}, 434--437 (1983)
\bibitem{U2} Urabe, T.: On quartic surfaces and sextic curves with singularities of type
$\widetilde E_8,\ T_{2,3,7},\ \widetilde E_{12}$.
Publ. Inst. Math. Sci. Kyoto Univ. {\bf 80}, 1185--1245 (1984)
\bibitem{U3} Urabe, T.: Singularities in a certain class of quartic surfaces and sextic curves
and Dynkin graphs. Proc. Vancouver Conf. Algebraic Geom., July 2-12, 1984. Providence, pp. 477--497 (1986)
\bibitem{Va} Varchenko, A. N.: Asymptotic of integrals and Hodge
structures. Modern Problems of Math., Vol. 22 (Itogi nauki
i tekhniki VINITI), Moscow, pp. 130--166 (1983)
\bibitem{Var1} Varchenko, A.~N.: On semicontinuity of the spectrum and an upper estimate for the number of singular points of a projective hypersurface. Sov. Math. Dokl. {\bf27}, 735--739 (1983);
    translation from Dokl. Akad. Nauk SSSR {\bf270}, no. 6, 1294--1297 (1983)
%\bibitem{Vi3} Viro, O. Ya.: Real algebraic plane curves: constructions with
%controlled topology. Leningrad Math. J. {\bf 1}, 1059--1134 (1990)
\bibitem{Wa1} Wahl, J.: Deformations of plane curves with nodes and cusps.
Amer. J. Math. {\bf 96}, 529--577 (1974)
\bibitem{Wa2} Wahl, J.: Equisingular deformations of plane algebroid curves.
Trans. Amer. Math. Soc. {\bf 193}, 143--170 (1974)
\bibitem{W1} Wall, C. T. C.: Geometry of quartic curves.
Math. Proc. Camb. Phil. Soc. {\bf 117}, 415--423 (1995)
\bibitem{W2} Wall, C. T. C.: Highly singular quintic curves.
Math. Proc. Camb. Phil. Soc. {\bf 119}, 257--277 (1996)
\bibitem{Wes1} Westenberger, E.: Existence of hypersurfaces with prescribed singularities. Commun. Algebra
{\bf31}, no. 1, 335--356 (2003)
\bibitem{Wes} Westenberger, E.: Real hypersurfaces with many simple singularities.
Rev. Mat. Complut. {\bf 18}, no. 2, 455--464 (2005)
\bibitem{Xu} Xu, G.:  Ample line bundles on smooth surfaces. J. Reine Angew. Math. {\bf469}, 199--209 (1995)
%Subvarieties of general hypersurfaces in projective spaces.
%J. Diff. Geom. {\bf 39}, 139--172 (1994)
\bibitem{ZL} Zaidenberg, M. G., Lin, V. Ya.: An irreducible simply connected algebraic curve in $\C^2$ is equivalent to a quasihomogeneous curve. Dokl. Akad. Nauk SSSR {\bf271}, no. 5, 1048--1052 (1983)
%\bibitem{ZO} Zaidenberg, M. G., Orevkov, S. Yu.: On rigid rational cuspidal plane curves.  Russ.  Math.  Surveys {\bf51}, 179--180 (1996)
\bibitem{Za0} Zariski, O.: On the Problem of Existence of Algebraic Functions of Two Variables Possessing a Given
Branch Curve. Amer. J. Math. {\bf51}, no. 2, 305--328 (1929)
\bibitem{Za1} Zariski, O.: Studies in equisingularity I-III. Amer. J. Math. {\bf 87}, 507--536, (1965);
Amer. J. Math. {\bf 87}, 972--1006 (1965); Amer. J. Math. {\bf 90}, 961--1023 (1968)
\bibitem{Za2} Zariski, O.: Algebraic surfaces, 2nd edn. Springer,
Heidelberg (1971)

\end{thebibliography}

